Rare decays of b hadrons

Rare decays of b hadrons provide a powerful way of identifying contributions from physics beyond the Standard Model, in particular from new hypothetical particles too heavy to be produced at colliders. The most relevant experimental measurements are reviewed and possible interpretations are briefly discussed.

==> DtauAndFit.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[bt]\centering
%\vskip -4em % due to subsection
%\hskip 0.05\textwidth
%\begin{minipage}{0.45\textwidth}
\includegraphics[height=0.4\textwidth]{rdrds_eps15.pdf}\hskip 0.02\textwidth
\includegraphics[height=0.4\textwidth]{FLNU-Sc1.pdf}
\caption{(left) Constraints on $R_D$ and $R_\Dstar$ from BaBar, Belle and LHCb. Plot courtesy of HFAG\cite{HFAG}. (right) Allowed regions in the $C_9^e$ versus $C_9^\mu$ plane. Figure from Ref.\cite{Descotes-Genon:2015uva}. The diagonal line marked ``LFU'' indicates values consistent with lepton universality, i.e. $C_9^\mu=C_9^e$.}\label{Fig:Dtaunu}\label{Fig:Fits}
%  \end{minipage}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> diffPreamble.tex <==
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

